Optimal Noise Adding Mechanisms for Approximate Differential Privacy

We study the (nearly) optimal mechanisms in $(\epsilon,\delta)$-approximate differential privacy for integer-valued query functions and vector-valued (histogram-like) query functions under a utility-maximization/cost-minimization framework. We characterize the tradeoff between $\epsilon$ and $\delta$ in utility and privacy analysis for histogram-like query functions ($\ell^1$ sensitivity), and show that the $(\epsilon,\delta)$-differential privacy is a framework not much more general than the $(\epsilon,0)$-differential privacy and $(0,\delta)$-differential privacy in the context of $\ell^1$ and $\ell^2$ cost functions, i.e., minimum expected noise magnitude and noise power. In the same context of $\ell^1$ and $\ell^2$ cost functions, we show the near-optimality of uniform noise mechanism and discrete Laplacian mechanism in the high privacy regime (as $(\epsilon,\delta) \to (0,0)$). We conclude that in $(\epsilon,\delta)$-differential privacy, the optimal noise magnitude and noise power are $\Theta(\min(\frac{1}{\epsilon},\frac{1}{\delta}))$ and $\Theta(\min(\frac{1}{\epsilon^2},\frac{1}{\delta^2}))$, respectively, in the high privacy regime.

==> abstract.tex <==

We study the (nearly) optimal mechanisms in $(\epsilon,\delta)$-differential privacy for integer-valued query functions and vector-valued (histogram-like) query functions under a utility-maximization/cost-minimization framework. We characterize the tradeoff between $\epsilon$ and $\delta$ in utility and privacy analysis for histogram-like query functions, and show that the $(\e,\delta)$-differential privacy is a framework not much more general than the $(\e,0)$-differential privacy and $(0,\delta)$-differential privacy in the context of $\ell^1$ and $\ell^2$ cost functions, i.e., minimum expected noise magnitude and noise power. In the same context of $\ell^1$ and $\ell^2$ cost functions,  we show the near-optimality of uniform noise mechanism and discrete Laplacian mechanism in the high privacy regime (as $(\e,\delta) \to (0,0)$). We conclude that in $(\epsilon,\delta)$-differential privacy,  the optimal noise magnitude and noise power are $\Theta(\min(\frac{1}{\epsilon},\frac{1}{\delta}))$ and $\Theta(\min(\frac{1}{\epsilon^2},\frac{1}{\delta^2}))$, respectively, in the high privacy regime.
% for $\ell^1$ and $\ell^2$ cost functions. The nearly optimality of the two simple mechanisms is proved by deriving a lower bound on the minimum cost using linear programming and duality. We show that the ratio of the upper bound (achieved by uniform noise mechanism and Laplacian mechanism) and the lower bound is upper bounded by a constant as $(\e,\delta) \to (0,0)$ for $\ell^1$ and $\ell^2$ cost functions. In particular, we show that for $(0,\delta)$-differential privacy, the uniform noise mechanism is nearly optimal, and the multiplicative gap from the optimal cost goes to one as $\delta \to 0$ for a general class of cost functions.





% In this paper, we first study the optimal noise-adding mechanism to preserve $(\e, \delta)$-differential privacy for a single integer-valued query function.

% 1) we study the case $(0,\delta)$ dp. The upper bound is given by uniform distribution, and the lower bound is the solution to a linear program with relaxed dp constraints, for which we can find the optimal solution. The optimality of candidate solution for the primal problem is proved by constructing dual variables for the the dual problem. By comparing the lower bound and upper bound, we have the following results

%    \begin{itemize}
%    	\item for $\ell^1$ cost function, the additive gap is upper bounded by a constant, as $\delta$ goes to zero.

%    	\item for $\ell^2$ cost function, the multiplicative gap is upper bounded by a constant, indeed the ratio goes to 1, (right?)  as $\delta$ goes to zero.

%    	\item for general cost function, the multiplicative gap is upper bounded by a constant in terms of the increasing rate of the cost function.
%    \end{itemize}



% 2) Next we study the general $(\epsilon, \delta)$ dp. There are two cases:

% \begin{itemize}
% 	\item $\epsilon >(?) \delta$.  The upper bound is given by a discrete variant of Laplacian mechanism.
% 	We prove that when $\delta \le \e^{2+a}$ for any positive number $a>0$, the multiplicative gap between the lower bound and the upper bound is upper bounded by a constant, for L1 and L2 cost functions. And I conjecture the same result holds for general momentum cost functions.


% 	\item $\epsilon < \delta$. The upper bound is given by uniform distribution. The lower bound is given by solving a linear program with relaxed DP constraints. We prove the optimality of primal variables by constructing the corresponding dual variables. We find that the multiplicative ratio of lower bound and upper bound is upper bounded by a constant, as $\delta$ goes to zero, for $\ell^1$ and $\ell^2$ cost functions. We conjecture maybe it also holds for all momentum cost functions.
% \end{itemize}


==> introduction.tex <==

%\subsection{Background and Motivation}

Differential privacy is a framework to quantify to what extent  individual privacy in a statistical database is preserved while releasing useful statistical information about the database \cite{DMNS06}. The basic idea of differential privacy is that the presence of any individual data in the database should not affect the final released statistical information   significantly, and thus it can give strong privacy guarantees against an adversary with arbitrary auxiliary information. For more background  and motivation of differential privacy, we refer the readers to the survey \cite{DPsurvey}.


The standard approach to preserve $\epsilon$-differential privacy for real-valued query function is to perturb the query output by adding random noise with Laplacian distribution. Recently, Geng and Viswanath \cite{GV13} show that under a general utility-maximization framework, for single real-valued query function, the optimal $\e$-differentially private mechanism is the staircase mechanism, which adds noise with staircase distribution to the query output. The optimality of the staircase mechanism is extended to the multidimensional setting for histogram-like functions in \cite{Geng13}, where the sensitivity of the query functions is defined using the $\ell^1$ metric as in \cite{DMNS06}. A relaxed notion of privacy, $(\e,\delta)$-differential privacy, was introduced by Dwork et al. \cite{DKMMN06}, and the standard approach to preserving   $(\e,\delta)$-differential privacy is to add Gaussian noise to the query output.

In this work, we study the (nearly) optimal mechanisms in $(\e,\delta)$-differential privacy for integer-valued query functions and vector-valued (histogram-like) query functions under a utility-maximization/cost-minimization framework, and characterize the tradeoff between $\epsilon$ and $\delta$ in utility and privacy analysis. $(\e,\delta)$-differential privacy is a relaxed notion of privacy, compared to the standard $\e$-differential privacy introduced in \cite{DMNS06}. $(\e,\delta)$-differential privacy includes as special cases:
\begin{itemize}
\item  $(\e,0)$-differential privacy;  in this standard setting, the optimal mechanism for a general cost minimization framework is the {\em staircase} mechanism as shown in \cite{GV13} and \cite{Geng13}. In the high privacy regime, the standard discrete Laplacian mechanism too performs well.
\item $(0,\delta)$-differential privacy; this setting requires that the total variation of the conditional probability distributions of the query output for neighboring datasets should be bounded by $\delta$. In this paper we show that the uniform noise distribution is  near-optimal in the $(0,\delta)$-differential privacy setting for a general class of cost functions.
\end{itemize}


While the $(\e,\delta)$-differential privacy setting is more general than the two special cases -- $(\e,0)$ and $(0,\delta)$-differential privacy -- our main result in this work is to show that it is only more general by {\em very little}; this is done in the context of $\ell^1$ and $\ell^2$ cost functions. We show the near-optimality of uniform noise and discrete Laplacian mechanisms in the high privacy regime (as $(\e,\delta) \to (0,0)$) for $\ell^1$ and $\ell^2$ cost functions.

The near-optimality of the two mechanisms (designed for the special cases of $(\epsilon,0)$ and $(0,\delta)$ differential privacy settings) is proved by demonstrating a uniform bound on the ratio between the costs of these two mechanisms and that of the optimal cost in the $(\epsilon,\delta)$ differential privacy setting in the high privacy regime, i.e.,  as $(\e,\delta) \to (0,0)$ for $\ell^1$ and $\ell^2$ cost functions.

%Further, we show that for $(0,\delta)$-differential privacy, the uniform noise mechanism is nearly optimal, and the multiplicative gap from the optimal cost goes to one as $\delta \to 0$ for a general class of cost functions.


\subsection{Summary of Our Results}

In this work we consider a very general model for integer-valued and vector-valued (histogram-like) query functions. Unlike previous works on $(\e,\delta)$-differential privacy (e.g., \cite{NTZ12}, \cite{KRSU10}, \cite{De12}), we impose no assumptions on the dataset model and properties of the query functions other than the global sensitivity, which is defined using the $\ell^1$ metric. We implicitly assume that the local sensitivity is equal to the global sensitivity. Due to the optimality of query-output independent perturbation as shown in \cite{GV13}, we consider query-output independent perturbation mechanisms.

We summarize our results in the following.  Let $V_{LB}$ denote the lower bound we derived for the cost under differential privacy constraint. Let  $V_{UB}^{\mbox{Lap}} $  and $V_{UB}^{\mbox{uniform}}$ denote the upper bounds for the cost achieved by discrete Laplacian mechanism and uniform noise mechanism. In this work, we show that
\begin{itemize}
	\item For integer-valued query functions,
	\begin{itemize}
		\item for $(0,\delta)$-differential privacy with the global sensitivity $\D = 1$, the uniform noise mechanism is optimal for all generic cost funtions,
		\item for $(0,\delta)$-differential privacy with arbitrary global sensitivity $\D$, $\lim_{\delta \to 0} \frac{V_{UB}^{\mbox{uniform}}}{V_{LB}} = 1$ for $\ell^1$ and $\ell^2$ cost functions,
		\item for $(\e,\delta)$-differential privacy with $\ell^1$ and $\ell^2$ cost functions, $\lim_{(\e,\delta) \to (0,0)} \frac{\min(V_{UB}^{\mbox{Lap}},V_{UB}^{\mbox{uniform}}  ) }{V_{LB}} \le C$ for some numerical constant $C$.
	\end{itemize}

	\item For vector-valued (histogram-like) query functions,
	\begin{itemize}
		\item  for $(0,\delta)$-differential privacy with the global sensitivity $\D = 1$, the multi-dimensional uniform noise mechanism  is optimal for $\ell^1$ and $\ell^2$ cost funtions,
		\item for $(0,\delta)$-differential privacy with arbitrary global sensitivity $\D$, $\lim_{\delta \to 0} \frac{V_{UB}^{\mbox{uniform}}}{V_{LB}} = 1$ for $\ell^1$ and $\ell^2$ cost functions,
		\item for $(\e,\delta)$-differential privacy with $\ell^1$ and $\ell^2$ cost functions, $\lim_{(\e,\delta) \to (0,0)} \frac{\min(V_{UB}^{\mbox{Lap}},V_{UB}^{\mbox{uniform}}  ) }{V_{LB}} \le C$ for some numerical constant $C$, which is independent of the dimension of the query function.
	\end{itemize}
\end{itemize}

We conclude that in $(\epsilon,\delta)$-differential privacy, the optimal noise magnitude and noise power are $\Theta(\min(\frac{1}{\epsilon},\frac{1}{\delta}))$ and $\Theta(\min(\frac{1}{\epsilon^2},\frac{1}{\delta^2}))$, respectively, in the high privacy regime, and naturally, the total cost grow linearly in terms of the dimension of the query output.






\subsection{Related Work}

Dwork et. al. \cite{DMNS06} introduce $\e$-differential privacy and show that the Laplacian mechanism, which perturbs the query output by adding random noise with Laplace distribution proportional to the global sensitivity of the query function, can preserve $\e$-differential privacy. In \cite{DMNS06}, it is shown that for histogram-like query functions, where the query output has multiple components and the global sensitivity is defined using the $\ell^1$ metric, one can perturb each component independently by adding the Laplacian noise to preserve $\e$-differential privacy.

Nissim, Raskhodnikova and Smith \cite{NRS07} show that for certain nonlinear query functions, one can improve the accuracy by adding data-dependent noise calibrated to the smooth sensitivity of the query function, which is based on the local sensitivity of the query function.
McSherry and Talwar \cite{McSherry07} introduce the \emph{exponential mechanism} to preserve $\e$-differential privacy for general query functions in an abstract setting, where the query function may not be real-valued.
Dwork et. al. \cite{DKMMN06} introduce $(\e,\delta)$-differential privacy and show that adding random noise with Gaussian distribution can preserve $(\e,\delta)$-differential privacy for real-valued query function. Hall, Rinaldo, and Wasserman \cite{Hall13} study how to preserve $(\e,\delta)$-differential privacy for releasing (infinite dimensional) functions, and show that adding Gaussian process noise to the released function can preserve  $(\e,\delta)$-differential privacy.
Kasiviswanathan and Smith \cite{Smith08} study $(\e,\delta)$-semantic privacy under a Bayesian framework. Chaudhuri and Mishra \cite{Chaudhuri06}, and Machanavajjhala et. al. \cite{Kifer08} propose different variants of the standard $\e,\delta$-differential privacy.


Ghosh, Roughgarden, and Sundararajan  \cite{Ghosh09} show that for a single count query with sensitivity $\D = 1$, for a general class of utility functions, to minimize the expected cost under a Bayesian framework the optimal mechanism to preserve $\e$-differential privacy is the geometric mechanism, which adds noise with geometric distribution. Brenner and Nissim  \cite{Nissim10}  show that for general query functions no universally optimal mechanisms exist. Gupte and Sundararajan \cite{minimax10} derive the optimal noise probability distributions for a single count query with sensitivity $\D = 1$ for minimax (risk-averse) users. \cite{minimax10} shows that although there is no universally optimal solution to the minimax optimization problem in \cite{minimax10} for a general class of cost functions, each solution (corresponding to different cost functions) can be derived from the same geometric mechanism by randomly remapping. Geng and Viswanath \cite{GV13} generalize the results of \cite{Ghosh09} and \cite{minimax10} to real-valued (and integer-valued) query functions with arbitrary sensitivity, and show that the optimal query-output independent perturbation mechanism is the staircase mechanism, which adds noise with a staircase-shaped probability density function (or probability mass function for integer-valued query function) to the query output. The optimality of the staircase mechanism is extended to the multidimensional setting for histogram-like functions in \cite{Geng13}, where the sensitivity of the query functions is defined using the $\ell^1$ metric as in \cite{DMNS06}.

Differential privacy for histogram query functions has been widely studied in the literature, e.g.,  \cite{Fang12,Hay10,geometry,Xu2012,Li10,NTZ12}, and many existing works use the Laplacian mechanism as the basic tool. For instance, Li et al. \cite{Li10} introduce the matrix mechanism to answer batches of linear queries over a histogram in a differentially private way with good accuracy guarantees. Their approach is that instead of adding Laplacian noise to the workload query output directly, the matrix mechanism will design an observation matrix which is the input to the database,  from perturbed output (using the standard Laplace mechanism)  estimate the histogram itself, and then compute the query output directly.  \cite{Li10} shows that this two-stage process will preserve differential privacy and increase the accuracy. Hay et al. \cite{Hay10} show that for a general class of histogram queries, by exploiting the consistency constraints on the query output, which is differentially private by adding independent Laplace noises, one can improve the accuracy while still satisfying differential privacy. These existing works study how to efficiently answer a set of linear queries on the histogram, while our work addresses the problem of releasing the histogram itself, which can be viewed as the worst-case query release (without knowing which linear queres will be asked).

Hardt and Talwar \cite{geometry} study the tradeoff between privacy and error for answering a set of linear queries over a histogram under $\epsilon$-differental privacy. The  error is defined as the worst  expectation of the $\ell^2$-norm of the noise. \cite{geometry} derives a lower bound for the error in the high privacy regime by using tools from convex geometry and Markov's inequality, and gives an upper bound by analyzing a differentially private mechanism, $K$-norm mechanism, which is an instantiation of the exponential mechanism and involves randomly sampling from a high dimensional convex body.  The lower bound given in \cite{geometry} depends on the volume of a convex body associated with the lineary query functions, and the lower bound  works for arbitrary linear query functions. In our problem setting, the linear query functions we are studying are the histogram function, which is a speical case of   \cite{geometry}  by setting $d = n$ and setting $F$ to be the identity map function. In this case, the lower bound given in \cite{geometry} is $\Omega(\frac{\sqrt{d}}{\epsilon})$\footnote{Note that for the $d$-dimensional $\ell^1$ unit ball, the volume is $\frac{2^d}{d!}$, and thus in Theorem 3.4 of \cite{geometry}, Vol$(K)^{1/d}= \Theta(\frac{1}{d})$.}, which matches our result, as we show that for $\epsilon$-differental privacy, in the high privacy regime, adding independent Laplacian noises to each component of the histogram is asymptotically optimal in the context of $\ell^1$ and $\ell^2$ cost functions.


Nikolov, Talwar and Zhang \cite{NTZ12} extend the result of \cite{geometry} on answering linear querys over a histogram to the case of  $(\e,\delta)$-differential privacy. Using tools from discrepancy theory, convex geometry and statistical estimation, they derive lower bounds and upper bounds of the error, which are within a multiplicative factor of $O(\log \frac{1}{\delta})$ in terms of $\delta$. Their bounds work for any set of linear query functions over a histogram, while in our work we study only the identity function, i.e., the query output is the histogram itself. Our result shows that in the high privacy regime (as $(\epsilon,\delta) \to (0,0)$), the optimal error scales as $\Theta(\min(\frac{1}{\epsilon},\frac{1}{\delta}))$ and $\Theta(\min(\frac{1}{\epsilon^2},\frac{1}{\delta^2}))$ for $\ell^1$ and $\ell^2$ cost functions, respectively. Therefore, our results significantly improve the bounds in \cite{NTZ12} in terms of $\epsilon$ and $\delta$ in the high privacy regime where both $\epsilon$ and $\delta$ go to zero.





Kasiviswanathan, Rudelson, Smith and Ullman \cite{KRSU10} derive lower bounds on the noise for releasing contingency tables under $(\e,\delta)$-differential privacy constraint, where the lower bounds depend on the size and structure of the database. %The difference between our work and \cite{KRSU10} is that the key factors in the lower bounds of \cite{KRSU10} are $n,k,d$, which are parameters of the dataset and contingency tables.
Our lower bounds are tighter and sharper than those of \cite{KRSU10} in terms of $\epsilon$ and $\delta$. For instance, in \cite{KRSU10}, for $(\e,\delta)$-differential privacy the lower bounds are proportional to $(1-\frac{\delta}{\epsilon})$, which are zero whenever $\delta = \epsilon$, while our results show that the lower bound is $\Theta(\min (\frac{1}{\epsilon}, \frac{1}{\delta}))$ as $(\epsilon,\delta) \to (0,0)$.

Anindya De \cite{De12}  studies lower  bound on the additive noise for Lipschitz query functions in $(\e,\delta)$-differential privacy which uses a different metric for the noise, and the lower bound depends on the size of the database. Jain, Kothari, and Thakurta \cite{Jain12} study how to preserve $(\epsilon,\delta)$-differential privacy for online learning algorithms, and show that the approximate differential privacy can be achieved by adding Gaussian noise to each component of the query output. They derive lower bounds on the noise, and the lower bounds can be viewed as an application of the composition theorem in \cite{DRV10} by Dwork, Rothblum, and Vadhan, which has been improved by Oh and Viswanath \cite{Oh13} recently. The difference of \cite{Jain12} and other related works from our work is that the global sensitivity of the query function is defined using $\ell^{\infty}$ metric in \cite{Jain12} and \cite{DRV10}, while in our work we use $\ell^1$ metric.




\subsection{Organization}

This paper is organized as follows. We formulate the utility-maximization/cost-minimization under the $(\e,\delta)$-differential privacy constraint for a single integer-valued query function  as a linear programming problem in Section \ref{sec:formulation}. In Section \ref{sec:zerodelta}, we study $(0,\delta)$-differential privacy, and show the nearly optimality of the simple uniform noise mechanism. In Section \ref{sec:epsilondelta}, we study the optimal mechanisms in $(\e,\delta)$-differential privacy, and show the optimality of uniform noise	mechanism and Laplacian mechanism in the regime $(\e,\delta) \to (0,0)$ in the context of $\ell^1$ and $\ell^2$ cost functions. In Section \ref{sec:zerodeltamulti}, we extend the results to the multidimensional setting for histogram-like query functions, where the query output is a vector of integers.

